Return of the Encoder: Maximizing Parameter Efficiency for SLMs

The dominance of large decoder-only language models has overshadowed encoder-decoder architectures, despite their fundamental efficiency advantages in sequence processing. For small language models (SLMs) - those with 1 billion parameters or fewer - our systematic analysis across GPU, CPU, and NPU platforms reveals that encoder-decoder architectures achieve 47% lower first-token latency and 4.7x higher throughput compared to decoder-only models on edge devices. These gains may be attributed to encoder-decoder's one-time input processing and efficient separation of understanding and generation phases. We introduce a novel knowledge distillation framework that enables encoder-decoder models to leverage capabilities from large scalable decoder-only teachers while preserving their architectural advantages, achieving up to 6 average performance points improvement across diverse tasks, with significant gains in asymmetric sequence tasks where input and output distributions can benefit from different processing approaches. When combined with modern advances like Rotary Positional Embeddings (RoPE) and Vision encoders, our systematic investigation demonstrates that encoder-decoder architectures provide a more practical path toward deploying capable language models in resource-constrained environments. Our findings challenge the prevailing trend toward decoder-only scaling, showing that architectural choices become increasingly crucial as parameter budgets decrease, particularly for on-device and edge deployments where computational efficiency is paramount.

==> backup.tex <==
\rui{Not sure if this is required, but people normally only put year in parentheses if the citation/author name is part of the sentence (also see guidance in Section 2.10. Citations and References from the ICML example paper: \url{https://media.icml.cc/Conferences/ICML2025/Styles/example_paper.pdf} ).Therefore, I changed similar citations to use citet for this purpose in the Introduction. Happy to change other citations in the rest of the paper if you want :) } -- \melfeki{thanks, Rui... That works for me.}

\rui{We mentioned both RoPE and ViT at the beginning but the rest of sentence seems to be only about vision. Not sure if we also want to mention RoPE's benefit as well.} --\melfeki{Rephrased the sentence.}


\rui{It's great to have this arch diagram to compare between enc-dec and dec-only. I am a bit confused whether we consider KV cache in the model design for this arch diagram. On the right side (decoder-only), it's mentioned that "reprocessing input for every out token". If I understand it correctly, this is without using KV cache, right? If we use KV cache, I guess the input doesn't need reprocessing because their key/value vectors are saved in the KV cache, which are used later by causal self-attention when generating each new output token. But in the following point, it's mentioned that "Growing KV cache per input tokens", which seems to suggest we are using KV cache here. Just want to make sure which case we are considering (using KV cache or not using KV cache), and it might be better to stick with one case for this diagram (or we explicitly specify the KV cache case for related bullet points?). But I might have missed something. Happy to discuss more if needed :) } \rui{It's related to my first point. With "quadratic growth", it looks like we are not using KV cache. Just want to double check :)} \rui{Not sure if "constant" latency is the right word to describe it, because as input length increases, the encoder part of enc-dec still needs to process longer input sequence, which takes more time (rather than simply constant), right? Also, the decoder part of enc-dec has cross-attention, which will cross attend to all the input tokens, whose complexity depends on the input length. Therefore, if I understand it correctly, it seems that the latency of encoder-decoder is not strictly constant with respect to the input length. But I understand that your main point is to emphasize that decoder-only has significantly longer latency. Just want to make sure that we choose words carefully if possible. Not sure if it's the right way to think about it. Happy to discuss more :) }--\melfeki{Rephrased it to answer your concern: “Encoder–decoder models only need to store the input’s encoded representation once, while decoder-only models must carry large K/V caches for every token at each layer, making encoder–decoder far more efficient for long inputs.”}


\rui{Just want to double check what we mean by "fixed-sized" representations "regardless of" input length. If I understand it correctly, there is one hidden-state vector for each input token as the output of the encoder. In other words, the output of encoder depends on the input length (i.e., longer input leads to longer encoder output). Or, do you mean the dim of each hidden-state vector is fixed? Not sure if I am overthinking about it, but just want to double check if possible :)} -- \melfeki{Added (while the sequence length varies with input)}

\rui{It looks like the total number of layers for enc-dec is 44 (=22+22 or =12+32), which is less than the total number of layers for dec-only (i.e., 48). It might be better to (briefly) explain the reason. Is it because the decoder-part of enc-dec has cross-attn sub-layers whereas decoder-only doesn't have them, which results in less total layers for enc-dec?} --\melfeki{Rephrased the paragraph for better explanation}

\rui{By "quadratic", I guess we are still talk about no KV cache. I feel that in most places of this paper, we are assuming no KV cache as I read more. Not sure if we want to explicitly mention it earlier in the paper. Even with KV cache, I guess enc-dec would have less memory footprint, because enc-dec only saves the hidden states from the last encoder layer, but decoder-only needs to save the K/V states from all the intermediate layers. Just want to mention it in case we want to be a bit more careful :) } -- \melfeki{Rephrased the entire paragraph to be more precise. Thanks for pointing that out.}

Our solution follows \cite{onpolicy} and involves careful sequence alignment strategies\rui{Do we want to say something like "Our solution follows Agarwal et al. (2024) but involves novel sequence alignment strategies that are carefully designed for distilling enc-dec models from decoder-only models"? In the original sentence, it sounds like we just use everything from Agarwal et al. (2024) without any novel contributions. It might be better to explicitly mention what our contributions are on top of Agarwal et al. (2024) :) }. For an input sequence $x$, we first generate output sequence $y$ using the student model. We structure the inputs distinctly: the teacher receives a concatenated sequence $[PAD]^{n_e} \circ x \circ y \circ [PAD]^{n_d}$, while the student model processes $x \circ [PAD]^{n_e}$ in the encoder and $[BOS] \circ y \circ [PAD]^{n_d}$ in the decoder\rui{It might be better to explain a bit what [PAD] and [BOS] are for better clarity. Probably many people would correctly understand them as padding token and beginning-of-sentence token, but might be still better to define any new notations}\rui{The same applies to $n_e$ and $n_d$ if possible.}. This arrangement ensures proper alignment through careful offset management, with teacher logits starting at position $(|x| + n_e - 1)$ \rui{also could define $|x|$ a bit if possible :) }and student logits coming directly from the decoder output.--\melfeki{Rewrote the paragraph}

\rui{might want to add a citation for reverse KL-divergence, e.g., \cite{onpolicy}} -- \melfeki{Cited above}

\rui{This figure comparing performance across model scales are very informative. But I feel that it's a bit too small to read. Might consider enlarging its legend, x/y-axis labels, etc. } --\melfeki{Space is a bit tight. Will see what I can do after I finish all modifications.}

\rui{To provide a holistic view with a global visual context, the original image is also resized to a low-resolution thumbnail image that matches the input resolution of the vision encoder~\cite{liu2024improved}.}  --\melfeki{Added}

\rui{feature alignment via LLaVA pretraining dataset~\cite{liu2023visual}, OCR understanding via UReader~\cite{ye2023ureader} and SynDoG~\cite{kim2022ocr},} --\melfeki{Added}
